WaveNets: Wavelet Channel Attention Networks

Channel Attention reigns supreme as an effective technique in the field of computer vision. However, the proposed channel attention by SENet suffers from information loss in feature learning caused by the use of Global Average Pooling (GAP) to represent channels as scalars. Thus, designing effective channel attention mechanisms requires finding a solution to enhance features preservation in modeling channel inter-dependencies. In this work, we utilize Wavelet transform compression as a solution to the channel representation problem. We first test wavelet transform as an Auto-Encoder model equipped with conventional channel attention module. Next, we test wavelet transform as a standalone channel compression method. We prove that global average pooling is equivalent to the recursive approximate Haar wavelet transform. With this proof, we generalize channel attention using Wavelet compression and name it WaveNet. Implementation of our method can be embedded within existing channel attention methods with a couple of lines of code. We test our proposed method using ImageNet dataset for image classification task. Our method outperforms the baseline SENet, and achieves the state-of-the-art results. Our code implementation is publicly available at https://github.com/hady1011/WaveNet-C.

==> tables/frequency_combination.tex <==

\begin{table}[htbp]
	\centering
	\caption{The results of using different numbers of frequency components on ImageNet with ResNet-50 backbone.}
	\label{combination}
	\begin{tabular}{ccc}
		\toprule
		Number    & Top-1 acc   & Top-5 acc  \\
		\midrule
		1   & 77.26     & 93.55\\
		2	& 78.40		& 94.07\\
		4	& 78.38		& 94.03\\
		8   & 78.33		& 94.06\\ 
		16 	& \textbf{78.52}  	& \textbf{94.14}\\
		32 	& 78.42  	& 94.10\\
		\bottomrule
	\end{tabular}
\end{table}



%\begin{table}[htbp]
%	\centering
%	\caption{The effects of different combinations of frequency components on the ImageNet dataset.}
%	\label{combination}
%	\begin{tabular}{ccc}
%		\toprule
%		Number    & Top-1 acc   & Top-5 acc  \\
%		\midrule
%		1   &  & \\
%		2	&  77.30 & 93.51\\
%		4	&  77.27 & 93.57\\
%		8   &  77.51 & 93.63\\ 
%		16 	&  77.17 & 93.53\\
%		32 	&  77.60 & 93.78\\
%		\bottomrule
%	\end{tabular}
%\end{table}

%\begin{table}[htbp]
%	\centering
%	\caption{The effects of different combinations of frequency components on the ImageNet dataset.}
%	\label{combination}
%	\begin{tabular}{ccc}
%		\toprule
%		Number    & Top-1 acc   & Top-5 acc  \\
%		\midrule
%		1   & 77.26 & 93.55\\
%		2	&  78.40 & 94.07\\
%		4	&  78.27 & 94.06\\
%		8   &  78.25 & 94.01\\ 
%		16 	&  78.26 & 94.12\\
%		32 	&  78.37 & 94.08\\
%		\bottomrule
%	\end{tabular}
%\end{table}

==> tables/instance_segmentation.tex <==

% \begin{table}[h]
% 	\centering
% 	\caption{Instance segmentation results of different methods using Mask R-CNN on COCO val 2017.}
% 	\label{segmentation}
% 	\setlength{\tabcolsep}{0.7mm}{\begin{tabular}{l|c|c|c|c|c|c}
% 		\toprule
% 		Method & AP & $AP_{50}$ & $AP_{75}$ & $AP_{S}$ & $AP_{M}$ &$AP_{L}$\\
% 		% & Training & Inference 
% 		\hline
% 		ResNet-50\ \ \   & 34.1 & 55.5 & 36.2 & 16.1 & 36.7 & 50.0\\
% 		SENet\ \ \  & 35.4 & 57.4 & 37.8 & 17.1 & 38.6 & \textbf{51.8}\\
% 		GCNet\ \ \  & 35.7 & 58.4 & 37.6 & N/A & N/A & N/A\\
% 		ECANet\ \ \  & 35.6 & 58.1 & 37.7 & 17.6 & 39.0 & \textbf{51.8}\\
% 		FcaNet (Ours)\ \ \  & \textbf{36.2} & \textbf{58.6} & \textbf{38.1} & \textbf{20.9} & \textbf{39.7} & 48.7\\
% 		\bottomrule

% 	\end{tabular}}
% \end{table}

\begin{table}[h]
	\centering
	\caption{Results of the instance segmentation task on COCO val 2017 over different methods using Mask R-CNN.}
	\label{segmentation}
	\begin{tabular}{lccc}
		\toprule
		Method & AP & $AP_{50}$ & $AP_{75}$ \\
		% & Training & Inference 
		\hline
		ResNet-50\ \ \   & 34.1 & 55.5 & 36.2 \\
		SENet\ \ \  & 35.4 & 57.4 & 37.8 \\
		GCNet\ \ \  & 35.7 & 58.4 & 37.6 \\
		ECANet\ \ \  & 35.6 & 58.1 & 37.7 \\
		FcaNet-TS\ \ \  & \textbf{36.2} & 58.6 & 38.1\\
        \rowcolor{tb_bg_color}
		WaveNet-C\ \ \ & \textbf{---} & 58.3 & 38.6 \\
		\bottomrule
	\end{tabular}
\end{table}

==> tables/object_detection.tex <==

\begin{table*}[htbp]
	\centering
	\caption{Results of the object detection task on COCO val 2017 over different methods.}
	\label{detection}
%<<<<<<< HEAD
%	\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
%		\hline
%		Method  & Detector & Parameters & FLOPs & AP & $AP_{50}$ & $AP_{75}$ & $AP_{S}$ & $AP_{M}$ &$AP_{L}$\\
%		% & Training & Inference 
%		\hline
%		ResNet50 & \multirow{8}{*}{Faster-RCNN} & \textbf{41.53 M}  & \textbf{215.51 G} &  36.4   & 58.2 & 39.2 & 21.8 & 40.0 & 46.2\\
%		SENet &  & 44.02 M & 215.63 G & 37.7 & 60.1 & 40.9 & 22.9 & 41.9 & 48.2\\
%		ECANet & & \textbf{41.53 M} & 215.63 G & 38.0 & 60.6 & 40.9 & 23.4 & 42.1 & 48.0\\
%		FcaNet (Ours)  &  & 44.02 M & 215.63 G & \textbf{39.0} & \textbf{61.1} & \textbf{42.3} & \textbf{23.7} & \textbf{42.8} & \textbf{49.6}\\
%		\cline{1-1}
%		\cline{3-10}
%		ResNet101 & & \textbf{60.52 M} & \textbf{295.39 G} &  38.7 & 60.6 &41.9 &22.7 &43.2 &50.4\\
%		SENet &  & 65.24 M & 295.58 G & 39.6 &62.0 &43.1 &23.7 &44.0 &51.4\\
%		ECANet & & \textbf{60.52 M} & 295.58 G & 40.3 & 62.9 & 44.0 & \textbf{24.5} & 44.7 &51.3\\
%		FcaNet (Ours)  &  & 65.24 M & 295.58 G & \textbf{41.2} & \textbf{63.3} & \textbf{44.6} & 23.8 & \textbf{45.2} & \textbf{53.1}\\
%		\hline
%		ResNet50 & \multirow{5}{*}{Mask-RCNN} & \textbf{44.17 M} & \textbf{261.81 G} & 37.2  & 58.9 & 40.3 & 22.2 & 40.7 & 48.0\\
%		SENet &  & 46.66 M & 261.93 G & 38.7 & 60.9 & 42.1 & 23.4 & 42.7 & 50.0\\
%		GCNet & & 46.69 M & 261.94 G & 39.4 & \textbf{61.6} & 42.4 & N/A & N/A & N/A\\
%		ECANet & & \textbf{44.17 M} & 261.93 G & 39.0 & 61.3 & 42.1 & \textbf{24.2} & 42.8 & 49.9\\
%		FcaNet (Ours)  &  & 46.66 M & 261.93 G & \textbf{40.3} & \textbf{62.0} & \textbf{44.1} & \textbf{25.2} & \textbf{43.9} & \textbf{52.0}\\
%		\hline
%=======
	\begin{tabular}{lccccccccc}
		\toprule
		Method  & Detector & Parameters & FLOPs & AP & $AP_{50}$ & $AP_{75}$ & $AP_{S}$ & $AP_{M}$ &$AP_{L}$\\
		% & Training & Inference 
		\hline
		ResNet-50 & \multirow{5}{*}{Faster-RCNN} & 41.53 M  & 215.51 G &  36.4   & 58.2 & 39.2 & 21.8 & 40.0 & 46.2\\
		SENet &  & 44.02 M & 215.63 G & 37.7 & 60.1 & 40.9 & 22.9 & 41.9 & 48.2\\
		ECANet & & 41.53 M & 215.63 G & 38.0 & 60.6 & 40.9 & 23.4 & 42.1 & 48.0\\
		FcaNet-TS  &  & 44.02 M & 215.63 G & \textbf{39.0} & 61.1 & 42.3 & 23.7 & 42.8 & 49.6\\
		\rowcolor{tb_bg_color}
		WaveNet-C  &  & 44.02 M & 215.63 G & \textbf{----} & 60.9 & 42.3 & 23.0 & 42.9 & 49.9\\
		\hline
		ResNet-50 & \multirow{7}{*}{Mask-RCNN} & 44.17 M & 261.81 G & 37.2  & 58.9 & 40.3 & 22.2 & 40.7 & 48.0\\
		SENet &  & 46.66 M & 261.93 G & 38.7 & 60.9 & 42.1 & 23.4 & 42.7 & 50.0\\
		GCNet & & 46.69 M & 261.94 G & 39.4 & 61.6 & 42.4 & - & - & -\\
		ECANet & & 44.17 M & 261.93 G & 39.0 & 61.3 & 42.1 & 24.2 & 42.8 & 49.9\\
		FcaNet-TS  &  & 46.66 M & 261.93 G & \textbf{40.3} & 62.0 & 44.1 & 25.2 & 43.9 & 52.0\\
		\rowcolor{tb_bg_color}
		WaveNet-C  &  & 44.02 M & 215.63 G & \textbf{----} & 60.9 & 42.3 & 23.0 & 42.9 & 49.9\\
		\bottomrule
	\end{tabular}
\end{table*}
